Minimization of Dynamical Systems over Monoids

Quantitative notions of bisimulation are well-known tools for the minimization of dynamical models such as Markov chains and ordinary differential equations (ODEs). In \emph{forward bisimulations}, each state in the quotient model represents an equivalence class and the dynamical evolution gives the overall sum of its members in the original model. Here we introduce generalized forward bisimulation (GFB) for dynamical systems over commutative monoids and develop a partition refinement algorithm to compute the coarsest one. When the monoid is $(\mathbb{R}, +)$, we recover probabilistic bisimulation for Markov chains and more recent forward bisimulations for nonlinear ODEs. Using $(\mathbb{R}, \cdot)$ we get nonlinear reductions for discrete-time dynamical systems and ODEs where each variable in the quotient model represents the product of original variables in the equivalence class. When the domain is a finite set such as the Booleans $\mathbb{B}$, we can apply GFB to Boolean networks (BN), a widely used dynamical model in computational biology. Using a prototype implementation of our minimization algorithm for GFB, we find disjunction- and conjunction-preserving reductions on 60 BN from two well-known repositories, and demonstrate the obtained analysis speed-ups. We also provide the biological interpretation of the reduction obtained for two selected BN, and we show how GFB enables the analysis of a large one that could not be analyzed otherwise. Using a randomized version of our algorithm we find product-preserving (therefore non-linear) reductions on 21 dynamical weighted networks from the literature that could not be handled by the exact algorithm.

==> proofs.tex <==
\section{Appendix: proofs}\label{sec:proofs}

%\begin{proof}[Proof of Theorem~\ref{thm:quant}]
%	Let $R$ be a GFB, pick $s_0 \in \MM^X$ and set $\hs_0 = \psi_R(s_0) \in \MM^{\calX_R}$. We next show that $\hs_k = \psi_R(s_k)$ by induction over $k \geq 0$. Since the base case $k = 0$ is true by construction, we can turn to the induction step. For $k \geq 0$, we obtain
%	\[
%	\hs_{k+1} = F_R(\hs_k) = F_R(\psi_R(s_k)) = \psi_R(F(s_k)) = \psi_R(s_{k+1}) ,
%	\]
%	where the second identity follows from the induction hypothesis, while the third identity follows from the definition of $F_R$ and the fact that $R$ is a GFB. Conversely, if $\hs_k = \psi_R(s_k)$ for all $k \geq 0$, we can conclude for $k = 0$ and arbitrary $s_0 \in \MM^X$ that
%	\[
%	\psi_R(F(s_0)) = \psi_R(s_1) = \hs_1 = F_R(\hs_0) = F_R(\psi_R(s_0)) ,
%	\]
%	thus showing that $R$ is a GFB.
%\end{proof}


%\begin{proof}[Proof of Theorem~\ref{thm:maximal}]
%	Fix arbitrary GFBs $\sim_1, \ldots, \sim_\nu \subseteq R$ and let $\calH_1, \ldots,$ $\calH_\nu$ be the corresponding partitions, i.e., $\calH_i = X_{\sim_i}$. Moreover, let $\sim_\ast := \big( \bigcup_{i = 1}^m \sim_i \big)^*$ and $\calH^\ast := X_{\sim_\ast}$, where the asterisk denotes transitive closure of a relation. At last, let $x_{i_{H^\ast}} \in H^\ast$ denote some representative of $H^\ast \in \calH^\ast$. With this, pick an arbitrary $H^\ast \in \calH^\ast$. By construction of $\calH^\ast$, there exist $x_0, \ldots,x_k \in X$ and $i_0,\ldots,i_{k-1} \in \{1,\ldots,\nu\}$ so that $\{x_0,\ldots,x_k\} = H^\ast$, $x_k = x_{i_{H^\ast}}$ and
%	$x_j \sim_{i_j} x_{j + 1}$ for all $0 \leq j \leq k - 1$. Moreover, for any $G^\ast \in \calH^\ast$ and $1 \leq i \leq \nu$, there exist (unique) $G^i_1,\ldots,G^i_{m_i} \in \calH_i$ such that $\biguplus_{l = 1}^{m_i} G^i_l = G^\ast$. Since $x_j \sim_{i_j} x_{j + 1}$ and $\calH_{i_j}$ is a GFB, we obtain
%	\begin{align*}
%		\operatorname*{\bigoplus}_{x_\iota \in G^\ast} f_{x_\iota} & = \operatorname*{\bigoplus}_{l = 1}^{m_{i_j}} \operatorname*{\bigoplus}_{x_\iota \in G^{i_j}_l} f_{x_\iota} \\
%		& = \operatorname*{\bigoplus}_{l = 1}^{m_{i_j}} \operatorname*{\bigoplus}_{x_\iota \in G^{i_j}_l} f_{x_\iota}[x_j / 0_\op][x_{j+1} / (x_j \op x_{j+1})] \\
%		& = \operatorname*{\bigoplus}_{x_\iota \in G^\ast} f_{x_\iota}[x_j / 0_\op][x_{j+1} / (x_j \op x_{j+1})]
%	\end{align*}
%	Since $\{x_0,x_1,\ldots,x_k\} = H^\ast$ and $x_k = x_{i_{H^\ast}}$, an application of the argument for all $0 \leq j \leq k - 1$ implies that $\operatorname*{\bigoplus}_{x_\iota \in G^\ast} f_{x_\iota}$ is equivalent to
%	\begin{align*}
%		\operatorname*{\bigoplus} \limits_{x_\iota \in G^\ast} f_{x_\iota} [x_k / 0_\oplus : x_k \in H^\ast, x_k \neq x_{i_{H^\ast}}] [x_{i_{H^\ast}} / \bigoplus \limits_{x_l \in H^\ast} x_l ]
%	\end{align*}
%	Since the choice of $G^\ast, H^\ast \in \calH^\ast$ was arbitrary, we infer that $\calH^\ast$ is a GFB.
%\end{proof}


%\begin{proof}[Proof of Theorem~\ref{thm:bin:fe}]
%	Let us assume first that $\calX_R$ is a GFB, pick an arbitrary $(x_i,x_j) \in R$ and pick the unique $C' \in \calX_R$ such that $x_i,x_j \in C'$. With this, define $s' := s[x_i \mapsto 0_\op][x_j \mapsto s_{x_i} \op s_{x_j}]$ for an arbitrary $s \in \MM^X$, where $s[x_k \mapsto b]_{x_k} = b$ and $s[x_k \mapsto b]_{x_l} = s_{x_l}$ for all $b \in \MM$ and $x_l \neq x_k$. Then, since $\op$ is commutative and associative and because  $\calX_R$ is a GFB, we have that
%	\begin{align}\label{eq:thm:bin:fe:2}
%		\operatorname*{\bigwedge} \limits_{C \in \calX_R } \Bigl( \bigoplus\limits_{x_i \in C }f_{x_i}(s)  = \bigoplus \limits_{x_i \in C } f_{x_i}(s') \Bigr).
%	\end{align}
%	Since the choice of $(x_i,x_j) \in R$ and $s \in \MM^X$ was arbitrary, we infer that $\Psi^{\calX_R}_{x_i,x_j}$ is valid. For the converse, let us assume that $\Psi^{\calX_R}_{x_i,x_j}$ holds true for all $(x_i,x_j) \in R$ and pick any two $s,s' \in \MM^X$ such that
%	\begin{align}\label{eq:thm:bin:fe}
%		\operatorname*{\bigwedge} \limits_{C \in \calX_R } \Bigl( \bigoplus\limits_{x_i \in C } s_{x_i} = \bigoplus \limits_{x_i \in C } s'_{x_i} \Bigr)
%	\end{align}
%	With this, pick for any $C \in \calX_R$ some arbitrary representative $x_{i_C} \in C$ and let $\hX = \{ x_{i_C} : C \in \calX_R \}$ be the set of all representatives. For any $(x_i,x_j) \in R$, define $s_{i \to j} := s[x_i \mapsto 0_\op, x_j \mapsto s_{x_i} \op s_{x_j}]$. With this, the fact that $\op$ is commutative and associative ensures the existence of a sequence $x_{i_1},x_{i_2},...,x_{i_k}$ for which $\hs = (((s_{i_1 \to i_2})_{ i_2 \to i_3}) \ldots)_{i_{k-1} \to i_k}$ is such that
%	\begin{align*}
%		\operatorname*{\bigwedge} \limits_{C \in \calX_R } \Bigl( \bigoplus\limits_{x_i \in C } s_{x_i} = \bigoplus \limits_{x_i \in C } \hs_{x_i} \Bigr) ,
%	\end{align*}
%	$\hs_{x_i} = 0_\op$ for all $x_i \notin \hX$ and $\hs_{x_{i_C}} = \bigoplus\limits_{x_i \in C } s_{x_i}$ for all $C \in \calX_R$. Since $\Psi^{\calX_R}_{x_{i_l},x_{i_{l+1}}}$ is valid for all $1 \leq l \leq k - 1$, we obtain
%	\[
%	\operatorname*{\bigwedge} \limits_{C \in \calX_R } \Bigl( \bigoplus\limits_{x_i \in C }f_{x_i}(s)  = \bigoplus \limits_{x_i \in C } f_{x_i}(\hs) \Bigr).
%	\]
%	A similar argument for $s'$ ensures that there is an $\hs'$ such that $\hs'_{x_i} = 0_\op$ for all $x_i \notin \hX$, $\hs'_{x_{i_C}} = \bigoplus\limits_{x_i \in C } s'_{x_i}$ for all $C \in \calX_R$ and
%	\begin{align*}
%		\operatorname*{\bigwedge} \limits_{C \in \calX_R } \Bigl( \bigoplus\limits_{x_i \in C } s'_{x_i} & = \bigoplus \limits_{x_i \in C } \hs'_{x_i} \Bigr) , \\
%		\operatorname*{\bigwedge} \limits_{C \in \calX_R } \Bigl( \bigoplus\limits_{x_i \in C }f_{x_i}(s') & = \bigoplus \limits_{x_i \in C } f_{x_i}(\hs') \Bigr) .
%	\end{align*}
%	Thanks to~(\ref{eq:thm:bin:fe}), we infer that $\hs = \hs'$. This, in turn, implies the desired relation~(\ref{eq:thm:bin:fe:2}), thus showing that $\calX_R$ is a  GFB if and only if $\Psi^{\calX_R}_{x_i,x_j}$ is valid for all $(x_i,x_j) \in R$.
%\end{proof}

%\begin{proof}[Proof of Theorem~\ref{thm:computesmaximal}]
%	Pick the largest (i.e., coarsest) GFB $\calH_\ast$ that refines $X_R$ using Theorem~\ref{thm:maximal}. With this, set $\calH_0 := X_R$ and define for all $k \geq 0$ and $H \in \calH_k$
%	\begin{align*}
%		R_k(H) & := \{(x_i,x_j) \in H \times H : x_i \neq x_j \Rightarrow \Psi^{\calH_k}_{x_i,x_j} \land \Psi^{\calH_k}_{x_j,x_i} \}  \\
%		\calH_{k+1} & := \bigcup_{H \in \calH_k} H / R^\ast_k(H) ,
%	\end{align*}
%	where $R^\ast_k(H)$ denotes the transitive closure of $R_k(H)$. By construction, $R_k(H)$ is reflexive and symmetric, thus implying $\operatorname*{\bigoplus} \limits_{x_i \in H} f_{x_i}(s) = \operatorname*{\bigoplus} \limits_{x_i \in H} f_{x_i}(\tilde{s})$ for all $s \in \MM^X$, $H \in \calH_k$, where
%	\begin{align*}
%		\tilde{s} = s[x_j \mapsto 0_\oplus : x_j \notin \hX_{k+1}][x_{i_{C'}} \mapsto \bigoplus_{x_j \in C'} s_{x_j} : C' \in \calH_{k+1}]
%	\end{align*}
%	and $x_{i_C} \in C$ is a representative of class $C \in \calH_{k+1}$, while $\hX_{k+1} = \{ x_{i_C} : C \in \calH_{k+1} \}$. (Note that $H \in \calH_k$, while $C \in \calH_{k+1}$ and $\hX_{k+1}$ is defined using $\calH_{k+1}$.) This implies that $R_k$ is transitive. Indeed, for any $(x_i,x_j),(x_j,x_k) \in R_k$ and $s' \in \MM^X$, the previous equation ensures for state $s := s'[x_i \mapsto 0_\op, x_k \mapsto s'_{x_i} \op s'_{x_k}]$ and any $H \in \calH_k$ that
%	\begin{align*}
%		\operatorname*{\bigoplus} \limits_{x_i \in H} f_{x_i}(s) = \operatorname*{\bigoplus} \limits_{x_i \in H} f_{x_i}(\tilde{s}') = \operatorname*{\bigoplus} \limits_{x_i \in H} f_{x_i}(\tilde{s}'')
%		= \operatorname*{\bigoplus} \limits_{x_i \in H} f_{x_i}(\tilde{s}''') ,
%	\end{align*}
%	where
%	\begin{align*}
%		\tilde{s}' & \! = \! s[x_l \! \mapsto \! 0_\oplus : x_l \notin \hX_{k+1}][x_{i_{C'}} \! \mapsto \! \bigoplus_{x_j \in C'} s_{x_j} : C' \in \calH_{k+1}] , \\
%		\tilde{s}'' & \! = \! s'[x_l \! \mapsto \! 0_\oplus : x_l \notin \hX_{k+1}][x_{i_{C'}} \! \mapsto \! \bigoplus_{x_j \in C'} s'_{x_j} : C' \in \calH_{k+1}] , \\
%		\tilde{s}''' & \! = \! s'[x_i \! \mapsto \! 0_\op, x_j \! \mapsto \! 0_\op, x_k \! \mapsto \! s'_{x_i} \op s'_{x_j} \op s'_{x_k}] .
%	\end{align*}
%	Hence, $R_k^\ast = R_k$ and the expression $H/R$ is indeed well-defined in Algorithm~\ref{algorithm}. Further, a proof by induction over $k \geq 1$ shows that a) $\calH_\ast$ is a refinement of $\calH_k$ and b) $\calH_k$ is a refinement of $\calH_{k-1}$. Since $\calH_\ast$ is a refinement of any $\calH_k$, it holds that $\calH_\ast = \calH_k$ if $\calH_k$ is a GFB partition. Since $X$ is finite, b) allows us to fix the smallest $k \geq 1$ with $\calH_k = \calH_{k-1}$. This, in turn, implies that $\calH_{k-1}$ is a GFB. To see the complexity statement, we note that the algorithm can perform at most $|X|$ refinements, while each iteration compares $\calO(|X|^2)$ pairs. For the decidability, instead, we first note that the finiteness of $\MM$ ensures the finiteness of $\op \subseteq \MM \times \MM$ and any $f_{x_i}  \subseteq \MM^X \times \MM$. Hence, checking
%	\[
%	\operatorname*{\bigwedge}\limits_{C \in \calH} \Bigl( \bigoplus\limits_{x_k \in C }f_{x_k} = \bigoplus\limits_{x_k \in C} f_{x_k} [x_i / 0_\oplus] [x_j / (x_i \oplus x_j)]	\Bigr)
%	\]
%	amounts to a finite number of checks over finite sets and is thus decidable.
%\end{proof}


%\begin{proof}[Proof of Theorem~\ref{thm:cont}]
%	See proof of Theorem~\ref{thm:cont:char}.
%\end{proof}


%\begin{proof}[Proof of Lemma~\ref{lem:log:counter}]
%We start by noting that $\psi_R(v_{x_1},v_{x_2}) = \log(v_{x_1}) + \log(v_{x_2})$ is an exact lumping because $\partial_t \psi_R(v) $ $= (v_{x_1}^{-1}, v_{x_2}^{-1}) \cdot (\partial_t v_{x_1} , \partial_t v_{x_2} )^T $ $= \psi_R(v)$. At the same time, the ODE discretization of the model is
%\begin{align*}%\label{eq:toy:euler}
%	f_{x_1} & = x_1 + \dt x_1 \log(x_2) , &
%	f_{x_2} & = x_2 + \dt x_2 \log(x_1) .
%\end{align*}
%Writing $h = \dt x_1 x_2 \log(x_1 x_2)  + \dt^2 x_1 x_2 \log(x_1) \log(x_2)$ for convenience, we observe that
%\begin{align*}
%	\!\!\!\!\log(f_{x_1}) \!+\! \log(f_{x_2})  \!&=  \log(f_{x_1} f_{x_2})
%	%\\& \
%	\ = \  \log\big(x_1 x_2 + h \big) \\
%	&  = \log(x_1 x_2) + (\partial \log)(x_1 x_2) h + 
%			\\ &\qquad\quad (\partial^2 \log)(x_1 x_2) \tfrac{h^2}{2} + \calO(\dt^3) \\
%	&  = \log(x_1 x_2) + \frac{h}{x_1 x_2} - \frac{h^2}{2 x^2_1 x^2_2} + \calO(\dt^3) \\
%	&  = \log(x_1 x_2) + \dt \log(x_1 x_2)  + 
%	\\ &\quad  \ \  \!\dt^2 \!\log(x_1\!) \!\log(x_2\!) \! - \!	 \dt^2 \!\tfrac{1}{2}\! \log(x_1 x_2\!)^2 \!\!+\! \calO(\dt^3) 
%\end{align*}
%Here, $\calO$ refers to \emph{big O} notation from numerical analysis, while the third identity follows from Taylor's theorem and from $\partial \log(x) = x^{-1}$ and $\partial^2 \log(x) = - x^{-2}$. Since the higher-order term $\dt^2 \log(x_1) \log(x_2)$ cannot be expressed in terms of $\log(x_1 x_2)$, we conclude that $\calX_R$ is not a GFB.
%\end{proof}



%\begin{proof}[Proof of Theorem~\ref{thm:cont:char}]
%	To improve readability, we write $\psi$ instead of $\psi_R$ in the present proof. Since $\op$ is twice differentiable by assumption, so is $\psi = (\psi_H)_{H \in \calX_R}$. For any $H \in \calX_R$, Taylor's theorem thus ensures
%	\begin{align*}
%		\psi_H(F(s)) &= \psi_H(s + \dt \Phi(s)) \\
%		& = \psi_H(s) + (\partial_s \psi_H)(s + \dt \Phi(s)) \cdot \dt \Phi(s) + \calO(\dt^2) \\
%		& = \psi_H(s) + \dt \cdot (\partial_s \psi_H)(s + \dt \Phi(s)) \cdot \Phi(s) + \calO(\dt^2)
%	\end{align*}
%	
%	%\paragraph*{First statement}
%	We begin by assuming that $\psi$ is an exact lumping. Then, with $\partial_t v(t) = \Phi(v(t))$, by~\cite{tomlin1997effect} the derivative of $t \mapsto \psi_H(v(t))$ can be written as a function of $\big(\psi_C(v(t))\big)_{C \in \calX_R}$. Since $v(0) \in \RE^X$ can be chosen arbitrarily, there is thus a function $\wp_H$ such that $\wp_H(\psi(s)) = (\partial_s \psi_H)(s + \dt \Phi(s)) \cdot \Phi(s)$ for all $s \in \RE^X$. Overall, we conclude for all $s \in \RE^X$
%	\begin{align*}
%		\psi_H(F(s)) & = \psi_H(s) + \dt \cdot \wp_H(\psi(s)) + \calO(\dt^2)
%	\end{align*}
%	Since $H \in \calH$ can be chosen arbitrarily, following the argumentation from the proof of Theorem~\ref{thm:bin:fe}, we infer that for all $(x_i,x_j) \in R$ with $x_i \neq x_j$ formula $\Psi^{\calX_R}_{x_i,x_j}$ is valid up to $\calO(\dt^2)$. For the converse, let us assume that for all $(x_i,x_j) \in R$ with $x_i \neq x_j$ formula $\Psi^{\calX_R}_{x_i,x_j}$ is valid up to $\calO(\dt^2)$. Then, Taylor's theorem yields as before
%	\begin{align*}
%		\psi_H(F(s)) & = \psi_H(s) + \dt \cdot (\partial_s \psi_H)(s + \dt \Phi(s)) \cdot \Phi(s) + \calO(\dt^2)
%	\end{align*}
%	With this and the validity of the aforementioned $\Psi^{\calX_R}_{x_i,x_j}$, the argumentation from the proof of Theorem~\ref{thm:bin:fe} ensures the existence of functions $(\wp_H)_{H \in \calX_R}$ over $\RE^{\calX_R}$ such that
%	\begin{align*}
%		\psi_H(F(s)) & = \psi_H(s) + \dt \cdot \wp_H(\psi(s)) + \calO(\dt^2)
%	\end{align*}
%	for all $H \in \calX_R$ and $s \in \RE^X$. Hence, with $\partial_t v(t) = \Phi(v(t))$, the derivative of $t \mapsto \psi_H(v(t))$ can be written as a function of $\big(\psi_C(v(t))\big)_{C \in \calX_R}$. Since $v(0) \in \RE^X$ can be chosen arbitrarily, we obtain that $\psi$ is an exact lumping. This completes the proof of Theorem~\ref{thm:cont:char}. We next turn to the proofs of 1) and 2) of  Theorem~\ref{thm:cont}. For 1), we note that $\Psi^{\calX_R}_{x_i,x_j}$ is valid up to $\calO(\dt^2)$ for all $(x_i,x_j) \in R$ when $R$ is a GFB. Instead, for 2) we observe that for a linear $\psi_R$ there are no higher-order terms, i.e., $\calO(\dt^2) = 0$. This two observations, combined with the foregoing discussion, yield statements 1) and 2).
%\end{proof}


%\begin{proof}[Proof of Corollary~\ref{cor:fde}]
%	Set $\op = +$ in Theorem~\ref{thm:cont}.
%\end{proof}

%\begin{proof}[Proof of Corollary~\ref{cor:prob:bis}]
%	The vector of transient probabilities of the Markov chain at time $t \geq 0$ satisfies the forward Kolmogorov equations $\partial_t \pi(t) = Q^T \pi(t)$. Moreover, by~\cite{DBLP:conf/popl/CardelliTTV16}, an equivalence relation $R$ over $X$ is an ordinary lumpability if and only if $R$ is an FDE the forward Kolmogorov equations. With this, Corollary~\ref{cor:fde} yields
%	%2) and
%	the equivalence of 1) and 2). The equivalence of 2) and 3), instead, is a well-known fact~\cite{BuchholzOrdinaryExact}.
%\end{proof}
%

